Mobile Foundation Model as Firmware

In today's landscape, smartphones have evolved into hubs for hosting a multitude of deep learning models aimed at local execution. A key realization driving this work is the notable fragmentation among these models, characterized by varied architectures, operators, and implementations. This fragmentation imposes a significant burden on the comprehensive optimization of hardware, system settings, and algorithms. Buoyed by the recent strides in large foundation models, this work introduces a pioneering paradigm for mobile AI: a collaborative management approach between the mobile OS and hardware, overseeing a foundational model capable of serving a broad spectrum of mobile AI tasks, if not all. This foundational model resides within the NPU and remains impervious to app or OS revisions, akin to firmware. Concurrently, each app contributes a concise, offline fine-tuned "adapter" tailored to distinct downstream tasks. From this concept emerges a concrete instantiation known as \sys. It amalgamates a curated selection of publicly available Large Language Models (LLMs) and facilitates dynamic data flow. This concept's viability is substantiated through the creation of an exhaustive benchmark encompassing 38 mobile AI tasks spanning 50 datasets, including domains such as Computer Vision (CV), Natural Language Processing (NLP), audio, sensing, and multimodal inputs. Spanning this benchmark, \sys unveils its impressive performance. It attains accuracy parity in 85\% of tasks, demonstrates improved scalability in terms of storage and memory, and offers satisfactory inference speed on Commercial Off-The-Shelf (COTS) mobile devices fortified with NPU support. This stands in stark contrast to task-specific models tailored for individual applications.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> fig-A100-Orin-22.tex <==
\begin{figure*}[t]
	% \vspace{0.6em}
	\centering
	\includegraphics[width=1\textwidth]{figs/comparison-2.pdf}
	%\vspace*{-.6cm}
	\caption{Performance comparison of TS-models on A100 and Orin.}
     %Note that the y-axis of subfigure(a) is logarithmic.
	\label{fig:eval-acc-comparison1}
	\vspace{-15pt}
\end{figure*}

==> fig-A100-Orin-Pixel.tex <==
\begin{figure}[t]
	% \vspace{0.6em}
	\centering
	\includegraphics[width=0.48\textwidth]{figs/A100_Orin_Pixel.pdf}
	%\vspace*{-.6cm}
	\caption{\yjl{Performance comparison of TS-models on three hardware platforms.}}
     %Note that the y-axis of subfigure(a) is logarithmic.
	\label{fig:eval-acc-comparison2}
	\vspace{-15pt}
\end{figure}

==> fig-NPU-operation-benefits.tex <==
\begin{figure}[t]
	% \vspace{0.6em}
	\centering
	\includegraphics[width=0.48\textwidth]{figs/NPU-operation-benefits.pdf}
	%\vspace*{-.6cm}
	\caption{Comparison of inference performance of 5 popular NN models on mobile chips: latency and energy.}
     %Note that the y-axis of subfigure(a) is logarithmic.
	\label{fig:eval-NPU-benefits}
	% \vspace{-1em}
\end{figure}

==> fig-cost-energy.tex <==
\begin{figure}[t]
	% \vspace{0.6em}
	\centering
	\includegraphics[width=0.48\textwidth]{figs/cost-energy.pdf}
	%\vspace*{-.6cm}
	\caption{Runtime cost on energy.}
     %Note that the y-axis of subfigure(a) is logarithmic.
	\label{fig:cost-energy}
	% \vspace{-1em}
\end{figure}

==> fig-cost-latency.tex <==
\begin{figure}[t]
	% \vspace{0.6em}
	\centering
	\includegraphics[width=0.48\textwidth]{figs/cost-latency.pdf}
	%\vspace*{-.6cm}
	\caption{Runtime cost on latency.}
     %Note that the y-axis of subfigure(a) is logarithmic.
	\label{fig:cost-latency}
	% \vspace{-1em}
\end{figure}

==> fig-hardware.tex <==
\begin{figure}[t]
	\begin{subfigure}{.245\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figs/orin-1-2.jpg}
		\caption{
			% \circleD{\color3}{T22}: 
            NVIDIA Jetson ORIN NX}
	\end{subfigure}
	\begin{subfigure}{.225\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figs/fig-hardware-pixel-2.pdf}
		\caption{
			% \circleE{\color4}{T33}: 
			Pixel 7 Pro smartphone}
	\end{subfigure}
	\caption{The snapshots of our two typical mobile devices.
		%\sys (full-data) denotes fine-tuning with all training samples.
		}
	\label{fig:hardware}
	\vspace{-12pt}
\end{figure}

==> fig-mobilefm-control.tex <==
\begin{figure*}[t]
	% \vspace{0.6em}
	\centering
	\includegraphics[width=0.8\textwidth]{figs/mobilefm-design-task-control.pdf}
	%\vspace*{-.6cm}
	\caption{MobileFM architecture: task contorl.}
     %Note that the y-axis of subfigure(a) is logarithmic.
	\label{fig:MobileFM-archi-control}
	% \vspace{-1em}
\end{figure*}

==> fig-operator-number.tex <==
\begin{figure}[t]
	% \vspace{0.6em}
	\centering
	\includegraphics[width=0.45\textwidth]{figs/operator-number.png}
	%\vspace*{-.6cm}
	\caption{The total number of operator types (ONNX).}
     %Note that the y-axis of subfigure(a) is logarithmic.
	\label{fig:operator-types}
	% \vspace{-1em}
\end{figure}

==> fig-peft-methods.tex <==
\begin{figure*}[t]
	% \vspace{0.6em}
	\centering
	\includegraphics[width=0.9\textwidth]{figs/peft_methods.png}
	%\vspace*{-.6cm}
	\caption{A Comprehensive measurement of peft methods.}
     %Note that the y-axis of subfigure(a) is logarithmic.
	\label{fig:peft-methods}
	% \vspace{-1em}
\end{figure*}

==> fig-peft-performance.tex <==
\begin{figure}[t!]
	% \vspace{0.6em}
	\centering
	\includegraphics[width=0.5\textwidth]{figs/peft_performance.pdf}
	%\vspace*{-.6cm}
	\caption{The tuning performance under varying peft settings.}
     %Note that the y-axis of subfigure(a) is logarithmic.
	\label{fig:peft_performance}
	% \vspace{-1em}
\end{figure}

==> fig-peft-settings.tex <==
\begin{figure*}[t]
	% \vspace{0.6em}
	\centering
	\includegraphics[width=0.9\textwidth]{figs/peft_settings.png}
	%\vspace*{-.6cm}
	\caption{A Comprehensive measurement of peft settings.}
     %Note that the y-axis of subfigure(a) is logarithmic.
	\label{fig:peft-methods}
	% \vspace{-1em}
\end{figure*}

==> fig-peft-time.tex <==
\begin{figure*}[t!]
	% \vspace{0.6em}
	\centering
	\includegraphics[width=0.95\textwidth]{figs/peft_time.pdf}
	%\vspace*{-.6cm}
	\caption{The convergence time under varying peft settings.}
     %Note that the y-axis of subfigure(a) is logarithmic.
	\label{fig:peft_time}
	% \vspace{-1em}
\end{figure*}

==> fig-peft-trainable.tex <==
\begin{figure*}[t!]
	% \vspace{0.6em}
	\centering
	\includegraphics[width=0.95\textwidth]{figs/peft_trainable.pdf}
	%\vspace*{-.6cm}
	\caption{The trainable parameter size under varying peft settings.}
     %Note that the y-axis of subfigure(a) is logarithmic.
	\label{fig:peft_trainable}
	% \vspace{-1em}
\end{figure*}

==> sec-benchmark.tex <==
\section{Benchmark and Setups}

\subsection{\benchmark: a Comprehensive Mobile AI Benchmark} \label{sec:benchmark}

% \input{fig-pervasive-tasks.tex}

\mwx{How the task-specific models are selected? Using what kind of criterizon? This is important.}

\benchmark is a comprehensive benchmark aimed to understand the impacts of DL models on the performance of mobile AI tasks.
It has the following advantages over existing AI benchmarks:

\textbf{Rich support} 
Table~\ref{tab:pervasive-tasks} summarizes AI applications across five different domains, encompassing a total of 35 tasks and 50 datasets on mobile devices. 
Thoroughly investigating AI applications covering various mobile scenarios is of paramount importance for advancing AI technologies and systems. 
We collected data from prominent conferences like MobiCom and MobiSys over the past five years, focusing on applications used on devices such as smartphones, cameras, headphones, smart vehicles, and laptop. 
These applications cover key softwares such as translation, input methods, camera/gallery, and voice assistants. 
The models we use come from two sources.
One is from open-source projects in prominent conference papers and achieve the best results by reproducing their code.
% We reproduced their code to achieve the SOTA performance.
The other is from Paperwithcode platform \yjl{[link]}, where we utilized the open-source code to obtain the best results.
Note that we opted for such performance by judiciously piching the traditional models with less than 1B parameters.

\textbf{Multimodal tasks}
mAIbench presents the performance of various modalities of AI tasks, including text, image, audio, and sensing data. 
Table~\ref{tab:pervasive-tasks} provides a comprehensive comprehension of the real-world environment by harnessing complementary information across these modalities.% a comprehensive understanding of our surroundings by leveraging complementary information from all these modalities.
Additionally, it aslo demonstrates multimodal tasks that involve the conversion between different modalities, such as audio, image caption and visual question answering. 
To this end, the multimodal learning aims to process and integrate data from several modalities, advancing towards more general-purpose AI.
This will also propel the further development of multimodal applications, thereby exploring more intriguing and valuable mobile application scenarios.
% These types of tasks continue to emerge with intriguing applications as larger models unveil new and interesting use cases.

\textbf{Pervasive applications} \benchmark encompassed a diverse array of Apps, including but not limited to entertainment, education, shopping, and more. 
This comprehensive investigation encompassed a diverse range of mobile applications, totaling over 40 Apps as shown in Table~\ref{tab:pervasive-tasks}. 
These findings underscore the ubiquitous presence of AI in the mobile app landscape, enhancing user experiences and streamlining convenience across various domains.

%   \end{tikzpicture}

% \input{subsec-bench-setup.tex}

% \input{subsec-bench-benchmark.tex}

==> sec-impl.tex <==
\section{Implementation and Setups}\label{sec:impl}

==> sec-measurement.tex <==
\subsection{Experimental Observations}\label{sec:measurement}
% Using 0.1\% data of full-set will enable BERT to perform on par on \texttt{AGNEWS} (0.6, 0.86), \texttt{YAHOO}(0.45, 0.66), \texttt{YELP} (0.27, 0.46), as well. While on \texttt{MNLI}, PET perform on par with CLS (0.48, 0.45). The Full-CLS are almost the same with Roberta-large.
%We emphasize necessity of big model \mwx{and its huge system cost} in Figure~\ref{fig:eval-model}.

Based on the FedFSL workflow presented above, we perform a set of early experiments on its performance.
The results highlight the two sides of a coin: a satisfactory model accuracy yet huge resource cost on clients.

\input{tab-eval-softlabel.tex}
\textit{Observation-1: FedFSL achieves satisfactory accuracy with scarce data labels; for which both pseudo labeling and prompt learning are indispensable.} 
Table~\ref{tab:eval-softlabel} shows the convergence accuracy of RoBERTa-large~\cite{liu2019roberta} on 4 popular NLP datasets\footnote{You can find a detailed description of the datasets in $\S$\ref{sec:eval-setup}.}.
With only 64 data labels (0.005\%--0.05\% of the total dataset), FedFSL achieves 85.8\%--97.0\% relatively convergence accuracy to the full-set fine-tuning that assumes all data samples are labeled.
The accuracy could be further boosted by involving more data labels.
Neither pseudo labeling nor prompt learning alone is enough to exhibit a usable accuracy.
With only one of them, the relative convergence accuracy is 40\%--74\%.
%under skewed labels distribution.
%Ours will bring less benefit under uniform distribution, while benefits still exists (from 58.1\% to 61.9\%).
Furthermore, the skewed label distribution challenges the task:
on \texttt{YELP-F}, a vanilla FedNLP method results in much higher accuracy when the labels are uniformaly distributed;
neverthelss, the challenge is mostly addressed by FedFSL that achieves satisfactory accuracy in both cases.

\input{fig-eval-model.tex}
\textit{Observation-2: FedFSL incurs huge system cost.}
Our experiments highlight the excessive system cost (Figure~\ref{fig:eval-model}), as against the commonsense that few-shot learning is usually fast and lightweight~\cite{fan2021federated, zhang2020revisiting, guha2019one, chen2019closer}.
For example, training RoBERTa-large on \texttt{AGNEWS} takes 3.3 hours to converge, 7.3 million Joules of energy, 68.4 GBs of network transmission, and 10.4 GB peak memory.
The cost is about 1.4$\times$ higher than a full-set supervised FedNLP process on the same model and dataset.
We then dive deeper into the implications behind and identify three challenges for a resource-efficient FedFSL system.
% Cost refers to energy consumption.

$\bullet$ \textbf{Orchestrating training and inference}
FedFSL has two coupled components: a federated learning runtime that continuously updates a global model; an inference runtime that keeps generating pseudo labels.
The two components must be paced harmoniously:
the inference runtime generating too few pseudo labels could slow down the training;
otherwise, generating too many pseudo labels could lead to resource waste or even excessive erroneous labels, especially when the global model is still weak.
A mechanism to orchestrate the two components must be dynamic to fit the model learning progress.

$\bullet$  \textbf{Prompt learning needs large NLP model.}
Compact NLP models have been proposed for mobile scenarios with acceptable accuracy degradation.
However, our experiments demonstrate that a large, fully-fledged foundation language model is demanded in FedFSL.
As shown in Figure~\ref{fig:eval-model}, on \texttt{MNLI} and \texttt{YELP-F}, a large RoBERTa-large model (24 transformer blocks) can reach 91\% and 88\% relative accuracy to full-set fine-tuning, while Bert-base (12 transformer blocks) can only obtain 45\% and 59\%.
The rationale is that a large language model also encodes rich knowledge for downstream tasks, from which hand-crafted prompts can better extract useful information within limited data labels.

\begin{comment}
Performance under various foundation models:
\mwx{Using 0.1\% data of full-set will enable BERT to perform on par on \texttt{AGNEWS} (0.6, 0.86), \texttt{YAHOO}(0.45, 0.66), \texttt{YELP} (0.27, 0.46), as well. While on \texttt{MNLI}, PET perform on par with CLS (0.48, 0.45). The Full-CLS are almost the same with Roberta-large.}
\end{comment}

$\bullet$ \textbf{Excessive on-device inference to obtain trustful pseudo labels.}
Pseudo labeling typically requires performing inference on all unlabeled data, from which the most confident/valuable ones can be selected for future training.
Note that the inference is not one-pass, as the model is continuously updated each round.
According to our experiments, up to 87.4\% of the total energy cost on clients is attributed to the inference.
As will be shown in $\S$\ref{sec:design-filter}, randomly filtering out a large portion of samples to speed up pseudo labeling will degrade accuracy significantly.

\begin{comment}
\cdq{Noted that} 
current pseudo labeling work selects ideal high-confidence labels from all unlabeled data.
This means inference on enormous unlabeled data is needed, which is not scalable in FL.
Related work has been widely researched in active learning~\cite{settles2009active}.
Manually annotating is costly and time-consuming.
Some samples are similar, annotating too much those similar samples would bring slight or even no benefit for subsequent training, thus wasting time and resource in vain.
What is worse, the label quality is hard to guarantee.
Naive dropping unlabeled data for pseudo labeling would harm statistical utility.
\end{comment}

==> sec-platform.tex <==
\section{The MobileFM Platform} \label{sec:platform}

Figure of MobileFM platform.

\textbf{MobileFM overview.}

\subsection{Measurement Methodology}

==> subsec-bench-benchmark.tex <==
\subsection{A Comprehensive Benchmark of Mobile AI Tasks}
\label{subsec:bkgnd-benchmark}

\input{fig-pervasive-tasks.tex}

% \input{fig-operator-number.tex}

% \input{fig-peft-figure.tex}

% 1, DL-driven mobile applications are becoming increasingly pervasive. (many mobile tasks)
% 任务数量多

% 2, The tasks of mobile applications are diverse and involve almost all modalities. (many modes of task input and output)
% 任务输入输出的模态种类多

% 3, The NN models that support these tasks are highly heterogeneous. (operators, architectures, size)
% 任务所需的模型多且“异构”（算子，结构，大小）

% 草稿1
% We perform comprehensive benchmarking measurements on mobile AI tasks that highlight the motivation to improve the generality of mobile devices and provide implications for the design of the mobile foundation model.
We perform comprehensive measurements on mobile AI tasks, highlighting the motivation to build a benchmark (\benchmark) for diverse mobile AI tasks while improving the generality of mobile devices.

\textbf{DL-driven mobile applications are diverse and increasingly pervasive.} 
% With the proliferation of mobile devices and the explosive growth of AI demand, DL-driven mobile applications have been deployed on common mobile devices such as smartphones, smart cameras, and vehicle systems, and become an integral part of our daily lives. 
% As shown in Table, an increasing number of mobile tasks will be deployed on mobile devices.
Table.X summarizes the currently supported mobile tasks in \benchmark, encompassing multiple modalities.  
Evaluating baseline performance for diverse mobile tasks across different modalities is crucial for building a comprehensive mobile AI ecosystem, as it facilitates optimization efforts for mobile operators and hardware.   
Among the myriad tasks executed on mobile terminals, we select 5 representative categories from a "market" perspective (36 tasks with 50 datasets in total).   
% These tasks are commonly deployed on widely-used mobile devices, such as smartphones, smart cameras, and vehicular systems.
These commonly encountered tasks often exhibit distinct input-output modalities (even within the same category) and are frequently deployed on widely-used mobile devices, such as smartphones, smart cameras, and vehicular systems.
As mobile devices continue to enhance their capabilities and the demand for AI explodes, more and more tasks will be deployed on mobile devices and become an integral part of our daily lives.

% \textbf{The tasks of mobile applications are diverse and involve almost all modalities.}
% The table shows the types of typical mobile applications belonging to the above-mentioned categories on a mobile device. 
% We mainly classify all task types into five categories. 
% As observed, even tasks of the same class do not have exactly the same types of input and output modalities, which implies that there are many types of input and output modalities for all applications.

\textbf{The NN models that support these tasks are highly heterogeneous.}
% Each mobile device typically needs to support more than one mobile application, and these applications are often not a single modality. 
% As shown in Table, taking a smartphone as an example, it may need to support emoji prediction, optical character recognition, keyword spotting, image/text-to-speech, and other applications simultaneously. 
% The execution of these applications typically requires different specific models, which have different sizes and heterogeneous architectures.
As observed in Table.X, nearly all mobility tasks require running on a specific task-specific model.
Specifically, the execution of all tasks in the table involves a total of 32 state-of-the-art (SOTA) task-specific models (different datasets of the same task may also utilize different task-specific models). 
Finding a universal model that can serve all tasks simultaneously is challenging due to variations in input-output modalities across different tasks, and even within the same task, different datasets may exhibit significant differences when evaluated using the same model.
Similar to how current mobile devices typically need to support multiple mobile applications, which often include multiple modalities, it is impractical to rely on a single model to cater to all these applications. 
For instance, in the case of smartphones, they may need to support applications like emoji prediction, optical character recognition, keyword recognition, image-to-speech, etc. 
Executing these applications often requires different specific models, which come in various sizes and heterogeneous NN architectures.


% \textbf{\textit{Implications:}}
% \textit{Due to the existence of specific inputs and outputs for training/inference on mobile tasks, specific models are currently designed for specific mobile tasks. 
% However, simply providing operator acceleration and hardware support for these specific models can only lead to modest improvements. 
% As more DL-driven tasks require deployment on mobile devices, the modality diversity of mobile devices makes it increasingly undesirable to design a specific architecture for each task. 
% To make practical mobile devices better able to support more mobile applications, it is necessary to re-design the general paradigm for mobile applications on devices.}


==> subsec-bench-setup.tex <==
\subsection{Benchmark Setup}
\label{subsec:setup}

% \textbf{\sys prototype}
% We have fully implemented the \sys prototype atop PEFT [ref] and PandaGPT [ref].
% PandaGPT is a popular multimodal framework, which can take multimodal inputs simultaneously and compose their semantics naturally.
% To support more mobile applications, we have enhanced the model by adding an encoder to support audio information and a decoder to generate multiple modalities, including audio and images. 
% Additionally, we have added a PEFT (Parameter-Efficient Fine-Tuning) module, which enables efficient fine-tuning of various functional components' parameters, thereby making it suitable for a wider range of downstream tasks.
% \yjl{Detail}

\noindent \textbf{Baselines}
We compare \sys to the traditional task-specific models customized for each individual task.
We evaluated the performance of \yjl{40} models and tasks on \yjl{50} datasets, as shown in Table~\ref{tab:pervasive-tasks}.
For example, ResNet200 is a popular CNN model pretrained on ImageNet dataset for image classification task;
RoBERTa is a transformer-based NLP model pretrained on SQuAD dataset for question and answer task.

\noindent \textbf{Few-shot setting}
We experiment with four representative tasks, including NLP task - Question Answering (QA), CV task - Image Classification, Audio task - Spoken Language Understanding (SLU), and multimodal task - Audio Captioning.
For each dataset, we follow prior work [ref] to randomly select gold labels. 
By default, the labels form a skewed distribution across clients to be more realistic to real-world situation
For each dataset, we generate 3 diﬀerent few-shot settings, on which we repeat the experiments and report the mean results.

\noindent \textbf{PEFT setting}
PEFT library [ref], describe the four PEFT techniques and the three hyper-parameters.

\noindent \textbf{Hardware}
As prior literature, our experiments are carried out in an emulation manner on a GPU server with 16x NVIDIA A100. 
The on-device inference latency, memory, and energy are obtained on \yjl{NVIDIA Jetson ORIN with 16G memory}. 
GPTQ is used to quantize \sys to evaluate its runtime cost.

\noindent \textbf{Operators}
operators counting tools (TFLite, onnx, pytorch)

==> subsec-design-training.tex <==
\subsection{Training details}
To achieve versatile performance in diverse mobile tasks, \sys is fine-tuned through various PEFT methods and strategies tailored to different config paths. 
For tasks going through backbone (Path 1,3), only LoRA parameters in backbones are activated while freezing encoder LoRA modules.
For discriminative tasks that only go through encoders (Path 2), the encoder LoRA modules will be activated.

During each training iteration, we compute the CrossEntropy loss from actual labels and predicted tokens, utilizing it to update the LoRA/linear parameters.

are added to attention modules in foundation backbone.

updating them while freezing other parameters.
% through CrossEntropy loss and predicted token feedback. 
 involve encoder fine-tuning using InfoNCE loss, specifically for transformer modules and the linear projection head.
Text-based generative tasks (Path 3) combine input, context, and descriptive language prompts with a task-specific description language, generating tokens via the model's tokenizer. 
The predicted feedback 
% Backbone training employs cross-entropy loss and the AdamW optimizer. The complete training setup involves specific strategies and configurations for different paths and tasks.


To achieve usable performance on different mobile tasks, we fine-tune \sys through different PEFT methods and tuning strategies.
Each config path has their specific tuning strategies, now we describe them as follows:



\paragraph{Complex multimodel tasks (Path 1)}
Though most of tasks will go through the whole modules (i.e., Path 1), we only add LoRA parameters to the attention modules of the backbone.
During each training iteration, we compute the CrossEntropy loss from actual labels and predicted tokens, utilizing it to update the LoRA parameters,  while remaining the other parameters frozen. 
% In the case of the AudioCaption task, our model is trained on the Clotho and AudioCaps datasets, involving fine-tuning with a learning rate ranging from 0 to 0.0005, sequence length set at 512, utilizing 8$\times$A100 GPUs, with an approximate training duration of 10.8 hours. For ImageCaption tasks, our model is trained on the MSCOCO'14 and Flickr8k datasets, utilizing 8$\times$A100 GPUs, with a training duration of approximately 51.6 hours.


% PandaGPT is a model designed to align multimodal encoders from ImageBind with large language models from Vicuna3. 
% The training data consists of 160k instances of image-language instruction-following data, where each instance includes an image and a multi-turn conversation. 
% To reduce the number of trainable parameters, PandaGPT focuses on training a linear projection matrix (f) to connect ImageBind's representation with Vicuna, and additional LoRA weights on Vicuna's attention modules. 
% The training objective is to optimize the parameters of the linear projection matrix and LoRA weights. 
% During training, the loss is computed based on the system responses. 
% Note that during the training process for specific modality, only relevant encoders are updated, while the other encoders remain frozen. 
% PandaGPT is trained on the image-language dataset for two epochs with a learning rate of 5e-4 and linear decay, using 8$\times$A100 40G GPUs, with a maximum sequence length for Vicuna-13B set to 400. The training process takes around 3.6--12 hours to complete.

\paragraph{Discriminative tasks (Path 2)}
% How to fine-tune imagebind for classification tasks?
% If the input is processed, describe it briefly, e.g., we use pre-processing progress in \cdq{refs} to get figure rectangles in object detection tasks\dots
Similar to language-vision models such as CLIP~\cdq{refs} and imagebind~\cdq{refs}, the encoder adopts contrastive representation learning for fine-tuning employing the InfoNCE loss~\cdq{refs}. 
To achieve parameter efficiency, we only train the additional LoRA weights on the transformer modules of encoders and the linear projection head of imagebind~\cdq{refs}.
% In the case of human activity recognition, we employ the HAR smartphone dataset~\cdq{refs} to fine-tune both the vision encoder and text encoder. 
% The fine-tuning process includes setting learning rate to 5e-5, batch size of 64, and low rank of 1. 
For more intricate tasks, such as object detection, we utilize a region proposal network to generate a set of object proposals~\cdq{ref Detic}. 
Subsequently, the image encoder and text encoder are employed to obtain classification results, enabling the implementation of a two-stage object detection approach.

\paragraph{Text-based generative tasks (Path 3)}
% The encoder takes text as input, formatted uniformly into a dictionary comprising input, context, and label components. 
% Notably, context may be omitted for specific tasks.
The input and context information, along with task-specific descriptive language prompts, are combined with a prompt, a task-specific description language, and then fed into the model's tokenizer alongside label components to generate tokens. 
Similar to path 1, backbones are trained using the cross-entropy loss function and the AdamW optimizer. 
% For all kinds of tasks, the training stage sets a learning rate of 3e-4, weight decay of 0.0, warmup steps at 100, lora r at 16, lora alpha at 16, lora dropout at 0.05, and a sequence length of 512, except for text summary, set at 5120. 
% Particularly, given the backbone's natural affinity for the English language, for the question and answering task of the tydiQA dataset, we perform preprocessing on the Arabic language data and incorporate task-specific prompts as inputs to the model. The training process utilizes 8$\times$A100 GPUs, with varying training\_data\_size * epoch of1800000 and a total training time of 12 hours.

% Various tasks are supported, including input word prediction, QA (SQuAD2.0 and TyDi QA), translation (wmt22 en-de), emoji prediction (tweet\_eval), text classification (ag\_news and SST2), grammatical error correction (JFLEG), text summary (CNN Daily Mail), and code documentation generation (CodeSearchNet). 
% The data is formatted as dictionaries with specific keys, and a task-specific description language is used as prompts. 
% The model's backbone, along with a decoder, is trained with the cross-entropy loss function and the AdamW optimizer. 
% The maximum sequence length for Vicuna-13B is 400, and training takes about 12--40 hours with 4--8$\times$A100 40G GPUs. 
% Training parameters, learning rate, weight decay, LoRA settings, and warmup steps are consistent across tasks, except for the Text summary task's higher max\_seq\_length of 5120. The model is trained in different environments, utilizing multiple Nvidia A100 GPUs for each task, with varying training\_data\_size * epoch and total training times.

\paragraph{Others (Path 4)}
\cdq{Is there any task now?}
Yes, diffusion and tts. 
\cdq{How to train diffusion model and TTS? (TODO)}

\begin{comment}
% 4 
(Experiments - Encoders for each modality)
During the training process, the audio and IMU encoders are updated, while the image and text encoders remain frozen. 

% 5.1. 
(Scaling the Image Encoder)
By varying the size of the image encoder and fixing the size of other modality encoders, we find  that better visual features lead to improved zero-shot performance for all modalities. 

% 5.2. 
(Training Loss and Architecture - Capacity of the audio and depth encoders)
The capacity of encoders have impact on the classification performance. A larger audio encoder improves performance for audio tasks. 
//while a smaller depth encoder improves performance for depth tasks, as the number of (image,
depth) pairs is small.
\end{comment}


==> subsec-eval-NPUanalysis.tex <==
\subsection{\sys on NPU: What-if Analysis}
\label{subsec:NPUanalysis}

% If our vision comes true that there's an NPU fully accelerates \sys, what kind of gains will it obtain? Latency and energy consumption compared to the task-specific models (which assume only running on CPU/GPU).

\input{fig-cost-whatif.tex}
\input{tab-whatif-npu.tex}

This subsection conducts a what-if analysis: if our vision comes true that there's an NPU fully accelerates \sys, what kind of gains will it obtain in terms of latency and energy?
% Figure~\ref{fig:what-if} illustrates the evaluation results.
As shown in Figure~\ref{fig:what-if}, we measure the latency and energy consumption of running task-specific models on CPU and NPU, and \sys only on CPU, which are deonted as BL (CPU), BL (NPU) and FM (CPU), respectively.
Then, based on the acceleration and energy efficiency results of the task-specific model running on NPU compared to CPU as presented in $\S$2.2, we computed the inference latency and energy consumption of \sys on NPU, which is deonted as FM (NPU).

As observed, \sys's inference latency and energy consumption on CPU are notably 13$\times$ and 11$\times$ higher than the task-specific model. 
\sys achieves an average latency of 0.48s and energy consumption of 1.3J on NPU, which are 11.1\% and 55.2\% lower than task-specific models on CPU. 
Furthermore, we delve into the architectural intricacies of \sys to analyze the latency breakdown performance in Table~\ref{tab:whatif-npu}. 
From this table, we observe that the latency optimization bottleneck for mobilefm lies in the time taken by the IMG-encoder and the generation of the first token by the backbone, which are approximately 2.1s and 6.3s, respectively. 
These components collectively account for 31\% and 93\% of \sys's average latency (6.8s in Figure~\ref{fig:cost-latency-energy}(a)).
However, after being accelerated by the NPU, the other components exhibit near real-time inference (less than 100ms), like audio classification and text-to-speech.
These achievements demonstrate that, with the aid of NPU accelerator, \sys can support AI invocations for all mobile applications with affordable runtime cost.





==> subsec-eval-llama2.tex <==
\subsection{MobileFM with LLaMA2}
\label{subsec:llama2}

choose a few tasks to try LLaMa2 as a comparison, and talk about the impact of the base model's capability improvement on the whole

==> tab-benchmark.tex <==
\begin{table*}[t]
\scriptsize
\caption{Benchmark results. G: generative task; C: classification task.}
\begin{tabular}{|l|l|l|l|l|l|r|r|}
    \hline
    Category                     & Task                          & Type & Dataset             & Model            & Metric                                                                   & \multicolumn{1}{l|}{Acc. in Paper}                                                           & \multicolumn{1}{l|}{Acc. Obtained}                                                            \\ \hline
                                 & input word prediction $\normalsize{\textcircled{\scriptsize{T1}}}\normalsize$         & G    & PTB                 & RNN              & Top-K Acc                                                                & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{FFFFFF} }}                         & \begin{tabular}[c]{@{}r@{}}Top-1: 17.14\%\\ Top-3: 27.64\%\\ Top-5: 32.70\%\end{tabular}      \\ \cline{2-8} 
                                 & QA                            & G    & SQuAD  v1.1         & MobileBERT       & EM,F1                                                                    & \begin{tabular}[c]{@{}r@{}}EM:82.9\\ F1:90.0\end{tabular}                                    & \begin{tabular}[c]{@{}r@{}}EM:82.498\\ F1:89.943\end{tabular}                                 \\ \cline{2-8} 
                                 & machine translation           & G    & wmt19 en-de         & transformer      & SacreBLEU                                                                & 42.7                                                                                         & 42.8322                                                                                       \\ \cline{2-8} 
                                 & emoji prediction              & C    & tweet\_eval (emoji) & roBERTa          & M-F1                                                                     & Val:24.7 Test:30.9                                                                           & \begin{tabular}[c]{@{}r@{}}Val:26.3175\\  Test:31.6\end{tabular}                              \\ \cline{2-8} 
    \multirow{-5}{*}{NLP}        & text classification           & C    & tweet\_topic\_multi & roberta-base     & M-F1                                                                     & 55.8                                                                                         & 55.7                                                                                          \\ \hline
                                 & object detection              & C    & COCO                & Libra-rcnn       & mAP                                                                      & 43                                                                                           & 42.7                                                                                          \\ \cline{2-8} 
                                 & image retrieval               & C    & Clothes Retrieval   & resnet50-arcface & recall@1                                                                 & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                & 90.18\%                                                                                       \\ \cline{2-8} 
                                 & super-resolution              & G    & Set5                & Real-ESRGAN      & \begin{tabular}[c]{@{}l@{}}PSNR\\ SSIM\end{tabular}                      & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                & \begin{tabular}[c]{@{}r@{}}PSNR: 28.0111\\ SSIM: 0.8248\end{tabular}                          \\ \cline{2-8} 
                                 & Image Segmentation            & G    & ADE20K              & deeplabv3plus    & mIoU                                                                     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                & 42.70\%                                                                                       \\ \cline{2-8} 
                                 & optical character recognition & C    & ICDAR 2015          & EAST             & \begin{tabular}[c]{@{}l@{}}Recall  \\ Precision  \\ F-score\end{tabular} & \begin{tabular}[c]{@{}r@{}}Recall: 0.7347 \\ Precision: 0.8357\\ F-score:0.7820\end{tabular} & \begin{tabular}[c]{@{}r@{}}Recall: 0.7723 \\ Precision: 0.8464 \\ F-score:0.8077\end{tabular} \\ \cline{2-8} 
    \multirow{-6}{*}{CV}         & Digit Classification          & C    & MNIST               & LeNet5x          & accuracy                                                                 & \cellcolor[HTML]{FFFFFF}                                                                     & 0.991                                                                                         \\ \hline
                                 & Automatic Speech Recognition  & G    & LibriSpeech         & CTC+attention    & WER                                                                      & 3.16                                                                                         & 3.16                                                                                          \\ \cline{2-8} 
                                 & Spoken Language Understanding & G    & SLURP               & CRDNN            & (scenario)accuracy                                                       & 81.73\%                                                                                      & 81.84\%                                                                                       \\ \cline{2-8} 
                                 & activity recognition          & C    & LibryParty          & RNN              & Precision                                                                & 0.9518                                                                                       & 0.9519                                                                                        \\ \cline{2-8} 
                                 & emotion recognition           & C    & IEMOCAP             & ECAPA-TDNN       & accuracy                                                                 & 65.70\%                                                                                      & 64.10\%                                                                                       \\ \cline{2-8} 
                                 & speaker recognition           & C    & Voxceleb 1          & Xvector + PLDA   & EER                                                                      & 3.23\%                                                                                       & 3.22\%                                                                                        \\ \cline{2-8} 
    \multirow{-6}{*}{Audio}      & keyword spotting              & C    & Speech command      & cnn-trad-fpool3  & Top-1 Acc                                                                & 88.20\%                                                                                      & 87.20\%                                                                                       \\ \hline
    Sensing                      & Human Activity Recognition    & C    & HAR                 & MLP              & accuracy                                                                 & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                                                & 97.70\%                                                                                       \\ \hline
                                 & Text-to-Speech                & G    & LJSpeech            & Transformer      & MCD                                                                      & 3.8                                                                                          & 3.26                                                                                          \\ \cline{2-8} 
                                 & Audio Captioning              & G    & Clotho              & Transformer      & BLEU-1                                                                   & 53.40\%                                                                                      & 52.10\%                                                                                       \\ \cline{2-8} 
    \multirow{-3}{*}{Multimodal} & Image Captioning              & G    & MSCOCO'14           & LSTM             & BLEU-1                                                                   & 71.80\%                                                                                      & 69.80\%                                                                                       \\ \hline
    \end{tabular}
\end{table*}

==> tab-tuning.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
    \scriptsize
    \begin{tabular}{ccccccccccc}
    \cline{1-3}
    \multicolumn{1}{|c|}{Tasks}                                                      & \multicolumn{1}{c|}{Adaptive foundation structure} & \multicolumn{1}{c|}{Tuning methods} & \cellcolor[HTML]{00B0F0}Trainable parameter ratio & \cellcolor[HTML]{00B0F0}Mobile memory usage (G) & \cellcolor[HTML]{00B0F0}Energy cost (KJ) & Training speed (it/s) & \cellcolor[HTML]{00B0F0}Tuning performance improvement (metrics) & \cellcolor[HTML]{FFC000}Performance gap (metrics) & \cellcolor[HTML]{FFC000}Training latency (hours) & \cellcolor[HTML]{FFC000}Total parameter (B) \\ \cline{1-3}
    \multicolumn{1}{|c|}{\cellcolor[HTML]{FFC000}}                                   & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{Lora}           &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                             \\ \cline{3-3}
    \multicolumn{1}{|c|}{\cellcolor[HTML]{FFC000}}                                   & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{prefix-tuning}  &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                             \\ \cline{3-3}
    \multicolumn{1}{|c|}{\cellcolor[HTML]{FFC000}}                                   & \multicolumn{1}{c|}{}                              & p-tuning                            &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                             \\
    \multicolumn{1}{|c|}{\multirow{-4}{*}{\cellcolor[HTML]{FFC000}Object Detection}} & \multicolumn{1}{c|}{\multirow{-4}{*}{Encoder}}     & prompt-tuning                       &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                             \\ \cline{1-2}
    Semantic Segmentation                                                            & Encoder                                            &                                     &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                             \\
    \cellcolor[HTML]{2972F4}Spoken Language Understanding (SLU)                      & Encoder + Backbone                                 &                                     &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                             \\
    keyword spotting                                                                 & Encoder + Backbone                                 &                                     &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                             \\
    \cellcolor[HTML]{FFC000}QA                                                       & Backbone                                           &                                     &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                             \\
    \cellcolor[HTML]{2972F4}input word prediction                                    & Backbone                                           &                                     &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                             \\
    \cellcolor[HTML]{2972F4}Human Activity Recognition (HAR)                         & Encoder                                            &                                     &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                             \\
    \cellcolor[HTML]{2972F4}Image/Text-to-Speech                                     & Decoder                                            &                                     &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                             \\
    \cellcolor[HTML]{2972F4}Audio/Text-to-Image Generation                           & Encoder + Decoder                                  &                                     &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                             \\
    \cellcolor[HTML]{2972F4}Text generation                                          & Backbone + Decoder                                 &                                     &                                                   &                                                 &                                          &                       &                                                                  &                                                   &                                                  &                                            
    \end{tabular}
\end{table*}

==> todo.tex <==
\mwx{term: unlabeled data}

\mwx{Curriculum Learning: from easy samples to difficult ones. Our system: from easy model to difficult ones.}

\mwx{cloud service or aggregator?}
